Optimal Scaling Results for Moreau-Yosida Metropolis-adjusted Langevin Algorithms

We consider a recently proposed class of MCMC methods which uses proximity maps instead of gradients to build proposal mechanisms which can be employed for both differentiable and non-differentiable targets. These methods have been shown to be stable for a wide class of targets, making them a valuable alternative to Metropolis-adjusted Langevin algorithms (MALA); and have found wide application in imaging contexts. The wider stability properties are obtained by building the Moreau-Yosida envelope for the target of interest, which depends on a parameter $\lambda$. In this work, we investigate the optimal scaling problem for this class of algorithms, which encompasses MALA, and provide practical guidelines for the implementation of these methods.

==> sections_revision/ergodicity.tex <==


\subsection{Ergodicity Properties of Proximal MCMC}
\label{sec:ergodicity}
The ergodicity results in \cite{pereyra2016proximal} can be extended to all proximal MCMC chains under sufficient conditions on $\lambda$ and the tail behaviour of the target $\pi$.

Let us denote the acceptance region of proximal MCMC by
\begin{align*}
    A(\bm{x}) := \{\bm{y}: \pi(\bm{x})q(\bm{x}, \bm{y})\leq \pi(\bm{y})q(\bm{y}, \bm{x})\},
\end{align*}
where $q$ is the proximal MCMC proposal in~\eqref{eq:proximal_proposal}. Following \cite{roberts1996exponential} we say that $A(\cdot)$ converges inwards in $q$ if
\begin{align}
    \label{eq:inward}
    \lim_{\norm{\bm{x}}\to \infty} \int_{A(\bm{x})\Delta I(\bm{x})}q(\bm{x}, \bm{y})\rmd \bm{y}=0,
\end{align}
where $I(\bm{x}):=\{\bm{y}: \norm{\bm{y}}\leq \norm{\bm{x}}\}$ is the region on points interior to $\bm{x}$ and $A(\bm{x})\Delta I(\bm{x})$ denotes the symmetric difference $A(\bm{x})\Delta I(\bm{x}) = (A(\bm{x})\cup I(\bm{x}))\setminus (A(\bm{x})\cap I(\bm{x}))$.

We can then extend the result of \cite[Theorem 4.1]{roberts1996exponential} to proximal MCMC:
\begin{theorem}
\label{theo:ergodicity}
Suppose that $c(\bm{x}) = \bm{x}+\frac{\delta}{2}\nabla G^\lambda(\bm{x})$ is the mean next candidate position for proximal MCMC. Assume that $A(\cdot)$ converges inwards in $q$ and that
\begin{align*}
  \eta := \lim\inf_{\norm{\bm{x}}\to \infty} (\norm{\bm{x}}-\norm{c(\bm{x})})>0,  
\end{align*}
then, the proximal MCMC chain is $V_s$-uniformly ergodic with $V_s(\bm{x})=e^{s\norm{\bm{x}}}$ and $s<2\delta \eta$.\fra{I'm not so sure this is the right range for $s$}
\end{theorem}
\begin{proof}
The proof is identical to that of \cite[Theorem 4.1]{roberts1996exponential} with $c(\bm{x}) = \bm{x}+\frac{\delta}{2}\nabla G(\bm{x})$ (i.e. the mean next candidate position for MALA) replaced by $c(\bm{x}) = \bm{x}+\frac{\delta}{2}\nabla G^\lambda(\bm{x})$ therein.
\end{proof}


We next focus on the one-dimensional class of distributions $\mathcal{E}(\beta, \gamma)$ introduced in \cite{roberts1996exponential}:
\begin{definition}[Class of distributions $\mathcal{E}(\beta, \gamma)$]
We say that the one-dimensional distribution $\pi$ belongs to $\mathcal{E}(\beta, \gamma)$ for $\gamma>0$ and $0<\beta<\infty$, if
\begin{align*}
    \pi(x)\propto \exp\left(-\gamma\vert x\vert^{\beta}\right),\qquad \vert x\vert > x_0
\end{align*}
for some $x_0>0$.
\end{definition}

As shown in \cite{pereyra2016proximal}, given a distribution $\pi\in\mathcal{E}(\beta, \gamma)$ with $\beta\geq 1$ ($G$ is not concave for distributions with $\beta<1$), its Moreau-Yoshida envelope $\pi_\lambda\in\mathcal{E}(\beta^{\prime}, \gamma^{\prime})$, where $\beta^{\prime}=\min(\beta, 2)$ and $\gamma^{\prime} = (2\lambda)^{-1}$ if $\beta>2$, $\gamma^{\prime} = \gamma$ if $1\leq\beta<2$ and in the case $\beta=2$ we have $\gamma^\prime\leq \gamma$, with $\gamma^\prime=\gamma$ only if $\lambda=0$ and $\gamma^\prime$ a decreasing function of $\lambda$ which decays as $(2+2\lambda)^{-1}$.


Therefore, if $1\leq \beta < 2$, the tail behaviour of $\pi_\lambda$ coincides with that of $\pi$, and the condition on $\eta$ in Theorem~\ref{theo:ergodicity} follows from the same arguments used for MALA \cite{roberts1996exponential}.
For light tails ($\beta>2$), $\pi_\lambda$ has at most Gaussian tails, and we have that for $\lambda\geq \delta/2$ $\eta=\delta/(2\lambda)>0$ while for $\delta/4<\lambda<\delta/2$ we have $\eta=2-\delta/(2\lambda)>0$. In the Gaussian case (i.e. $\beta=2$), the condition on $\eta$ is satisfied for all $\gamma^{\prime}$ such that $\gamma^{\prime}\delta <2$, or, equivalently, if $\delta<4(1+\lambda)$.


==> sections_revision/extra_experiment.tex <==
To further investigate the scaling of proximal MALA to other non-differentiable densities, we empirically study the case  where the sequence of targets is given by: $x^d \in \rset^d$,
\begin{equation}
\label{eq:def_l2_l1_numerics}
\pi_d^{\mathrm{ GL }}(x^d) = \prod_{i=1}^d \exp(-g(x^d_i)) , \quad g(x)=\abs{x} + x^2/2 ,
\end{equation}
which, like the Laplace distribution in $0$, is non-differentiable but convex. The study of such a potential is motivated by Bayesian inverse problems considered in \cite{pereyra2016proximal,durmus2018efficient}, for which the posterior distribution arises from Gaussian observations and sparsity-induced priors like the Laplace distribution. The posterior then has the form (up to a multiplicative constant) $x^d \mapsto \exp(-\Vert y^d - \mathbf{A} x^d \Vert - c_r \sum_{i=1}^d \vert x_i \vert )$.

For this choice of target \eqref{eq:def_l2_l1_numerics}, the proposal of proximal MALA is given for any $d\in \nsets$, $k\in \nset$ and $i \in
\iint{1}{d}$,
\begin{equation} Y^d_{k+1,i} = \parenthese{1- \frac{\sigma_d^2}{2\lambda_d} } X^d_{k,i} + \frac{\sigma_d^2}{2\lambda_d}\parenthese{ (X^d_{k,i}-\sgn(X^d_{k,i}))\indicatorDD{|X^d_{k,i}| \geq \lambda_d} - \lambda_d X^d_{k,i}} + \sigma_d Z^d_{k+1,i},
\end{equation}
where $(Z^d_{k+1,i})_{k\in \nset}$ is a sequence of standard normal random variables. We then repeated the same experiments as for the Laplace distribution. The results are shown in \Cref{fig:mixed_mala,fig:mixed_pmala,fig:mixed_general_main}.
From these figures it is clear that the same scaling holds, i.e. choosing $\sigma_d^2 = \ell/d^{2\alpha}$, $\lambda = \sigma_d^{2m}r/2$ with $\alpha = 1/3$, $r \geq 0$.
%It can be rewritten as follows,
%\begin{equation}
%    Y_{k+1} = X^d_{k,i} - \frac{\sigma_d^2}{2} \parenthese{X^d_{k,i} + \sgn(X^d_{k,i})} \indicatorDD{|X^d_{k,i}| \geq \lambda_d}
%    - \frac{\sigma^2_d}{2} \frac{1 + \lambda_d}{\lambda_d} X^d_{k,i} \indicatorDD{|X^d_{k,i}| < \lambda_d}.
%\end{equation}
%This corresponds to using a \textit{pseudo-}proximal operator $\text{\textit{pseudo-}}\prox^{\lambda}_g(x)=(x-\sgn(x)\lambda)\indicatorDD{|x|\geq \lambda } - \lambda x$.
\begin{figure}
\centering
\begin{tikzpicture}[every node/.append style={font=\tiny}]
%\node (img1) {\includegraphics[width = 0.4\textwidth]{laplace_scaling_mala.pdf}};
%\node[below=of img1, node distance = 0, yshift = 1.2cm] {$d$};
%\node[left=of img1, node distance = 0, rotate = 90, anchor = center, yshift = -1cm] {$a_d(\ell, r)$};
\node (img1) {\includegraphics[width = 0.4\textwidth]{mixed_ar_general.pdf}};
\node[below=of img1, node distance = 0, yshift = 1.2cm] {$\ell$};
\node[left=of img1, node distance = 0, rotate = 90, anchor = center, yshift = -1cm] {$a_d(\ell, r)$};
\node[right=of img1, node distance = 0, xshift = -0.7cm] (img3) {\includegraphics[width = 0.4\textwidth]{mixed_esjd_general.pdf}};
\node[below=of img3, node distance = 0, yshift = 1.2cm] {$a_d(\ell, r)$};
\node[left=of img3, node distance = 0, rotate = 90, anchor = center, yshift = -1cm] {$\textrm{ESJD}_d$};
\end{tikzpicture}
\caption{Proximal MALA for the target \eqref{eq:def_l2_l1_numerics} and $m=3, r=2$, with $\sigma^2=\ell/d^{2\alpha}$ and $\alpha=1/3$.  Left: acceptance rate as a function of $\ell$ for increasing dimension $d$; Right: $\textrm{ESJD}_d$ as a function of the acceptance rate $a_d(\ell, r)$.}
\label{fig:mixed_general_main}
\end{figure}
%From \Cref{fig:mixed_mala,fig:mixed_pmala,fig:mixed_general_main}, we obtain the same scaling in
%$\alpha=1/3$ and similar expected squared jumping distance curves as to the Laplace case, even though we
%cannot obtain the results theoretically with our theorems.


==> sections_revision/laplace_integrals.tex <==
\subsection{Integrals for moment computations}
\label{app:integrals}
We distinguish the case $m=1/2$ and $m\geq1$ since the integration bounds significantly differ in these two cases. For values between $1/2$ and $1$ the integrals are not finite. 
The expectations below are obtained by integrating w.r.t. $x$ and using a Taylor expansion about $\sigma=0$ to obtain the leading order terms. Using the Lagrange form of the remainder for the Taylor expansions, we find that the remainder terms are all of the form $\sigma^{1/\alpha+1}f(\gamma(\sigma, z))/(1/\alpha+1)!$ where $\gamma(\sigma, z)$ is a point between the limits of integration w.r.t. $x$ and $f:x\mapsto p(x)e^{-x}$, where $p$ is a polynomial.
Therefore, using the boundedness of the remainder and Lebesgue's dominated convergence theorem, the integrals w.r.t. $z$ of the remainder terms all converge to 0.


\subsubsection{First Moment}


\paragraph{Case (a):} $m=1/2$

Let us consider $\phi_d^1$ first. For $r\geq \sigma$, we have
\begin{align*}
A_1\cap B_1 &=\begin{cases}
0\leq x\leq \frac{\sigma r}{2}\qquad\textrm{if } 0\leq z\leq \frac{\sigma}{2}\\
0\leq x\leq \left(\frac{\sigma r}{2}-\sigma z\right)\left(1-\frac{\sigma}{r}\right)^{-1}\qquad\textrm{if } \frac{\sigma}{2}\leq z\leq \frac{ r}{2}\\
-\sigma z\left(1-\frac{\sigma}{r}\right)^{-1}\leq x\leq \frac{\sigma r}{2}\qquad\textrm{if } \frac{\sigma}{2}- \frac{r}{2}\leq z\leq 0\\
\end{cases},
\end{align*}
and, similarly, 
\begin{align*}
A_1\cap B_2 &=\begin{cases}
0\leq x\leq \frac{\sigma r}{2}\qquad\textrm{if } -\frac{r}{2}\leq z\leq \frac{\sigma}{2}-\frac{r}{2}\\
0\leq x\leq -\sigma z\left(1-\frac{\sigma}{r}\right)^{-1}\qquad\textrm{if } \frac{\sigma}{2}-\frac{r}{2}\leq z\leq 0\\
-\left(\frac{\sigma r}{2}+\sigma z\right)\left(1-\frac{\sigma}{r}\right)^{-1}\leq x\leq \frac{\sigma r}{2}\qquad\textrm{if } \frac{\sigma}{2}-r\leq z\leq - \frac{r}{2}\\
\end{cases},
\end{align*}
and
\begin{align*}
A_1\cap (B_1 \cup B_2) &=\begin{cases}
0\leq x\leq \frac{\sigma r}{2}\qquad\textrm{if } -\frac{r}{2}\leq z\leq \frac{\sigma}{2}\\
0\leq x\leq \left(\frac{\sigma r}{2}-\sigma z\right)\left(1-\frac{\sigma}{r}\right)^{-1}\qquad\textrm{if } \frac{\sigma}{2}\leq z\leq \frac{r}{2}\\
-\left(\frac{\sigma r}{2}+\sigma z\right)\left(1-\frac{\sigma}{r}\right)^{-1}\leq x\leq \frac{\sigma r}{2}\qquad\textrm{if } \frac{\sigma}{2}-r\leq z\leq - \frac{r}{2}\\
\end{cases}.
\end{align*}
The above gives
\begin{align*}
\expe{\left(\frac{\sigma}{r}X-\sigma Z\right)\indicator{A_1}{X}\indicator{B_1}{X, Z}} &= \frac{1}{2\sqrt{2\uppi}}\int_{ \sigma/2}^{r/2}e^{-z^2/2}\left[\frac{\sigma^2}{2}(2z^2-rz)+\dots\right]\rmd z\\
&+ \frac{1}{2\sqrt{2\uppi}}\int_{ \sigma/2-r/2}^{0}e^{-z^2/2}\left[-\frac{\sigma^2}{2}(2z^2+2rz)+\dots\right]\rmd z+o(1),\\
\expe{\left(2X-\frac{\sigma}{r}X+\sigma Z\right)\indicator{A_1}{X}\indicator{B_2}{X, Z}} &= \frac{1}{2\sqrt{2\uppi}}\int_{ \sigma/2-r/2}^{0}e^{-z^2/2}\left[\frac{\sigma^3}{6r}(z^3r+3z^2)+\dots\right]\rmd z\\
&+ \frac{1}{2\sqrt{2\uppi}}\int_{ \sigma/2-r}^{-r/2}e^{-z^2/2}\left[-\frac{\sigma^3}{24}(4r^3+12r^2z+12r+12rz^2+4z^3+24z+\frac{12z^2}{r}) +\dots\right]\rmd z+o(1),
\end{align*}
and
\begin{align*}
&\mathbb{E}\left[\left(\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\left(\frac{2\sigma}{r}-\frac{\sigma^2}{r^2}\right)X-\left(1-\frac{\sigma}{r}\right)\sigma Z\right)^2\right)\indicator{A_1}{X}\indicator{B_1\cup B_2}{X, Z}\right]\\
&\qquad\qquad =\frac{1}{2\sqrt{2\uppi}}\int^{ \sigma/2}_{-r/2}e^{-z^2/2}\left[\frac{\sigma^2}{4}(2z^2+rz)+\dots\right]\rmd z\\
&\qquad\qquad +\frac{1}{2\sqrt{2\uppi}}\int_{ \sigma/2}^{r/2}e^{-z^2/2}\left[\frac{\sigma^2}{4}(-2z^2+rz)+\dots\right]\rmd z\\
&\qquad\qquad +\frac{1}{2\sqrt{2\uppi}}\int_{ \sigma/2-r}^{-r/2}e^{-z^2/2}\left[\frac{\sigma^2}{2}\ 0+\dots\right]\rmd z.
\end{align*}
%For $0<r< \sigma$, we have, 
%\begin{align*}
%A_1\cap B_1 &=\begin{cases}
%0\leq x\leq \frac{\sigma r}{2}\qquad\textrm{if } \frac{\sigma}{2}-\frac{r}{2}\leq z\leq \frac{r}{2}\\
%0\leq x\leq-\sigma z\left(1-\frac{\sigma}{r}\right)^{-1}\qquad\textrm{if } 0\leq z\leq \frac{\sigma}{2}-\frac{ r}{2}\\
%\left(\frac{\sigma r}{2}-\sigma z\right)\left(1-\frac{\sigma}{r}\right)^{-1}\leq x\leq \frac{\sigma r}{2}\qquad\textrm{if }  \frac{r}{2}\leq z\leq \frac{\sigma}{2}\\
%\end{cases},
%\end{align*}
%and, similarly, 
%\begin{align*}
%A_1\cap B_2 &=\begin{cases}
%0\leq x\leq \frac{\sigma r}{2}\qquad\textrm{if } \frac{\sigma}{2}-r\leq z\leq 0\\
%0\leq x\leq -\left(\frac{\sigma r}{2}+\sigma z\right)\left(1-\frac{\sigma}{r}\right)^{-1}\qquad\textrm{if } -\frac{r}{2}\leq z\leq \frac{\sigma}{2}-r\\
%-\sigma z \left(1-\frac{\sigma}{r}\right)^{-1}\leq x\leq \frac{\sigma r}{2}\qquad\textrm{if } 0\leq z\leq \frac{\sigma}{2} - \frac{r}{2}\\
%\end{cases},
%\end{align*}
%and
%\begin{align*}
%A_1\cap (B_1 \cup B_2) &=\begin{cases}
%0\leq x\leq \frac{\sigma r}{2}\qquad\textrm{if } \frac{\sigma}{2}-r \leq z\leq\frac{r}{2}\\
%0\leq x\leq -\left(\frac{\sigma r}{2}+\sigma z\right)\left(1-\frac{\sigma}{r}\right)^{-1}\qquad\textrm{if } -\frac{r}{2}\leq z\leq \frac{\sigma}{2}-r\\
%\left(\frac{\sigma r}{2}-\sigma z\right)\left(1-\frac{\sigma}{r}\right)^{-1}\leq x\leq \frac{\sigma r}{2}\qquad\textrm{if } \frac{r}{2}\leq z\leq \frac{\sigma}{2}\\
%\end{cases}.
%\end{align*}
%The above gives
%\begin{align*}
%\expe{\left(\frac{\sigma}{r}X-\sigma Z\right)\indicator{A_1}{X}\indicator{B_1}{X, Z}} &= \frac{1}{2\sqrt{2\uppi}}\int_{ \sigma/2-r/2}^{r/2}e^{-z^2/2}\left[-\frac{\sigma^2}{2}rz+\dots\right]\rmd z\\
%&+ \frac{1}{2\sqrt{2\uppi}}\int^{ \sigma/2-r/2}_{0}e^{-z^2/2}\left[\sigma^2z^2+\dots\right]\rmd z\\
%&+ \frac{1}{2\sqrt{2\uppi}}\int_{r/2}^{\sigma/2}e^{-z^2/2}\left[-\sigma^2z^2+\dots\right]\rmd z,\\
%\expe{\left(2X-\frac{\sigma}{r}X+\sigma Z\right)\indicator{A_1}{X}\indicator{B_2}{X, Z}} &= \frac{1}{2\sqrt{2\uppi}}\int_{ \sigma/2-r}^{0}e^{-z^2/2}\left[\frac{\sigma^2}{4}(r^2+2rz)+\dots\right]\rmd z\\
%&+ \frac{1}{2\sqrt{2\uppi}}\int_{ -r/2}^{\sigma/2-r}e^{-z^2/2}\left[\frac{\sigma^2}{2}(r^2+2rz) +\dots\right]\rmd z\\
%&+ \frac{1}{2\sqrt{2\uppi}}\int_{ 0}^{\sigma/2-r/2}e^{-z^2/2}\left[\frac{\sigma^2}{2}(r^2+2rz) +\dots\right]\rmd z,
%\end{align*}
%and
%\begin{align*}
%&\mathbb{E}\left[\left(\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\left(\frac{2\sigma}{r}-\frac{\sigma^2}{r^2}\right)X-\left(1-\frac{\sigma}{r}\right)\sigma Z\right)^2\right)\indicator{A_1}{X}\indicator{B_1\cup B_2}{X, Z}\right]\\
%&\qquad\qquad =\frac{1}{2\sqrt{2\uppi}}\int^{ r/2}_{\sigma/2-r}e^{-z^2/2}\left[\frac{\sigma^2}{4}(2z^2+rz)+\dots\right]\rmd z\\
%&\qquad\qquad +\frac{1}{2\sqrt{2\uppi}}\int_{ \sigma/2}^{r/2}e^{-z^2/2}\left[\frac{\sigma^2}{4}(2z^2+rz)+\dots\right]\rmd z\\
%&\qquad\qquad +\frac{1}{2\sqrt{2\uppi}}\int_{ r/2}^{\sigma/2}e^{-z^2/2}\left[\sigma^2 z^2+\dots\right]\rmd z.
%\end{align*}
For $\phi_d^2$, we have
\begin{align*}
A_3 \cap C_1=\begin{cases}
\sigma^2/2-\sigma z \leq x\leq \sigma^2/2-\sigma z +\sigma r/2\qquad\textrm{if } z<\sigma/2 -  r/2\\
\sigma r/2 < x\leq \sigma^2/2-\sigma z +\sigma r/2\qquad\textrm{if } \sigma/2 -  r/2\leq z\leq \sigma/2
\end{cases},
\end{align*}
and
\begin{align*}
\expe{\left(\frac{\sigma^2}{2}-\sigma Z\right)\indicator{A_3}{X}\indicator{C_1}{X, Z}} 
&=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2 -  r/2}e^{-z^2/2}\left[-\frac{\sigma^2}{2}rz+\frac{\sigma^3}{8}r(rz-4z^2+2)+...\right]\rmd z\\
&+\frac{1}{2\sqrt{2\uppi}}\int_{\sigma/2 -  r/2}^{\sigma/2} e^{-z^2/2}\left[\sigma^2z^2+\frac{\sigma^3}{2}z(z^2-2-rz)+...\right]\rmd z.
\end{align*}
Similarly, we obtain
\begin{align*}
A_3\cap C_2=\begin{cases}
\sigma^2/2-\sigma z-\sigma r/2\leq x\leq \sigma^2/2-\sigma z\qquad\textrm{if } z< \sigma/2- r\\
\sigma r/2< x\leq \sigma^2/2-\sigma z\qquad\textrm{if } \sigma/2- r< z<
	\sigma/2 - r/2
\end{cases}
\end{align*}
and
\begin{align*}
\expe{\left(2X-\frac{\sigma^2}{2}+\sigma Z\right)\indicator{A_3}{X}\indicator{C_2}{X, Z}}
&=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2- r}e^{-z^2/2}\\
&\qquad\qquad\left[-\frac{\sigma^2}{4}(r^2+2zr)-\frac{\sigma^3}{24}r (2 r^2 + 9 r z + 12 z^2-6)+...\right]\rmd z\\
&+\frac{1}{2\sqrt{2\uppi}}\int_{\sigma/2- r}^{\sigma/2-r/2}e^{-z^2/2}\\
&\qquad\qquad\left[-\frac{\sigma^2}{4}(r^2+2zr)+\frac{\sigma^3}{24}(6 r + 2 r^3 + 3 r^2 z + 4 z^3)+...\right]\rmd z.
\end{align*}
Finally, 
\begin{align*}
A_3\cap (C_1\cup C_2)=\begin{cases}
\sigma r/2\leq x\leq \sigma r/2+\sigma^2/2-\sigma z\qquad\textrm{if } \sigma/2- r\leq z\leq \sigma/2\\
-\sigma r/2+\sigma^2/2-\sigma z< x\leq \sigma r/2+\sigma^2/2-\sigma z\qquad\textrm{if } z< \sigma/2-  r
\end{cases},
\end{align*}
and
\begin{align*}
&\expe{\left(\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{\sigma}{r}X+\left(1-\frac{\sigma}{r}\right)\left(\frac{\sigma^2}{2}-\sigma Z\right)\right)^2\right)\indicator{A_3}{X}\indicator{C_1\cup C_2}{X, Z}}\\
&\qquad\qquad=\frac{1}{2\sqrt{2\uppi}}\int_{\sigma/2- r}^{\sigma/2}e^{-z^2/2}\left[-\frac{\sigma^2}{2r}(z^3+2rz^2)+\frac{\sigma^3z}{48r^2}(48r^2+48r+8z^2+24r^3z-24r^2z^2+12r^2z-8rz^2)...\right]\rmd z\\
&\qquad\qquad+\frac{1}{2\sqrt{2\uppi}}\int ^{ \sigma/2- r}_{-\infty}e^{-z^2/2}\left[\frac{\sigma^2}{2}rz+\frac{\sigma^3}{12}(6rz^2-r^2z-2r)+...\right]\rmd z.
\end{align*}
For $\phi_d^3$, we have, in the case $r\geq \sigma$,
\begin{align*}
A_1\cap B_3&=\begin{cases}
0\leq x\leq \frac{\sigma r}{2}\qquad\textrm{if }  z> \frac{r}{2}\\
\left(\frac{\sigma r}{2}-\sigma z\right)\left(1-\frac{\sigma}{r}\right)^{-1}< x\leq \frac{\sigma r}{2}\qquad\textrm{if } \frac{\sigma}{2}\leq z\leq \frac{ r}{2}
\end{cases},\\
A_1\cap B_4&=\begin{cases}
0\leq x\leq \frac{\sigma r}{2}\qquad\textrm{if } z< \frac{\sigma}{2}- r\\
0\leq  x<\left(\frac{\sigma r}{2}-\sigma z\right)\left(1-\frac{\sigma}{r}\right)^{-1}\qquad\textrm{if } \frac{\sigma}{2}- r\leq z\leq -\frac{ r}{2}
\end{cases};
\end{align*}
from which we obtain
\begin{align*}
&\expe{\left(\frac{\sigma}{r}X-\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{\sigma}{r}X -\sigma Z+\frac{\sigma^2}{2}\right)^2\right)\indicator{A_1}{X}\indicator{ B_3}{X, Z}} \\
&\qquad\qquad=\frac{1}{2\sqrt{2\uppi}}\int_{ r/2}^{+\infty}e^{-z^2/2}\left[-\frac{\sigma^2}{8}rz+\frac{\sigma^3}{48}(r^2z-r)+...\right]\rmd z\\
&\qquad\qquad+\frac{1}{2\sqrt{2\uppi}}\int_{ \sigma/2}^{r/2}e^{-z^2/2}\left[-\frac{\sigma^2}{2r}z^3+\frac{\sigma^3}{48r^2}(12r^2z^3-16rz^4+24rz^2-56z^3)...\right]\rmd z,\\
&\expe{\left(2X-\frac{\sigma}{r}X+\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{\sigma}{r}X -\sigma Z-\frac{\sigma^2}{2}\right)^2\right)\indicator{A_1}{X}\indicator{ B_4}{X, Z}} \\
&\qquad\qquad=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2- r}e^{-z^2/2}\left[\frac{\sigma^2}{8}(2r^2+3rz)-\frac{\sigma^3}{48}(4r^3+5r^2z+7r)+...\right]\rmd z\\
&\qquad\qquad+\frac{1}{2\sqrt{2\uppi}}\int^{-r/2}_{\sigma/2- r}e^{-z^2/2}\left[\frac{\sigma^2}{2}\left(\frac{r^2}{2}+\frac{z^3}{r}-\frac{5rz}{4}\right)+\frac{\sigma^3}{48r^5}(-4r^8+19r^7z+17r^6-24r^6z^2-48r^5z-4z^3r^5+16r^4z^4+56r^3z^3)...\right]\rmd z.
\end{align*}
\fral{fill in $\phi_d^3$ for case 2}
Finally, consider $\phi_d^4$ and $A_3 \cap  C_4=\left\lbrace z<\frac{\sigma}{2}- r, \frac{\sigma r}{2}<x\leq \frac{\sigma^2}{2 }-\sigma z -\frac{\sigma r}{2}\right\rbrace$, then
\begin{align*}
    \expe{\left(2X-\frac{\sigma^2}{2}+\sigma Z\right)\indicator{A_3}{X}\indicator{ C_4}{X, Z}}
&=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2- r}e^{-z^2/2}\left[\frac{\sigma^3}{6}
(r+z)^3+ \dots\right]\rmd z.
\end{align*}



\paragraph{Case (b):} $m\geq 1$


Let us consider $\phi_d^1$ first. Since we have, for $r\geq \sigma^{-2(m-1)}$,
\begin{align*}
A_1\cap (B_1\cup B_2)&=\begin{cases}
0\leq x\leq \frac{\sigma^{2m}r}{2}\qquad\textrm{if } -\frac{\sigma^{2m-1} r}{2}\leq z\leq \frac{\sigma}{2}\\
0\leq x\leq \left(\frac{\sigma^{2m}r}{2}-\sigma z\right)\left(1-\frac{1}{\sigma^{2(m-1)}r}\right)^{-1}\qquad\textrm{if } \frac{\sigma}{2}\leq z\leq \frac{\sigma^{2m-1} r}{2}\\
\left(-\frac{\sigma^{2m}r}{2}-\sigma z\right)\left(1-\frac{1}{\sigma^{2(m-1)}r}\right)^{-1}\leq x\leq \frac{\sigma^{2m}r}{2}\qquad\textrm{if } \frac{\sigma}{2}-\sigma^{2m-1} r\leq z\leq -\frac{\sigma^{2m-1} r}{2}\\
\end{cases},
\end{align*}
and, for $0\leq r< \sigma^{-2(m-1)}$
\begin{align*}
A_1\cap (B_1\cup B_2)&=\begin{cases}
0\leq x\leq \frac{\sigma^{2m}r}{2}\qquad\textrm{if } -\sigma^{2m-1} r+\frac{\sigma}{2}\leq z\leq \frac{\sigma^{2m-1} r}{2}\\
0\leq x\leq \left(-\frac{\sigma^{2m}r}{2}-\sigma z\right)\left(1-\frac{1}{\sigma^{2(m-1)}r}\right)^{-1}\qquad\textrm{if } -\frac{\sigma^{2m-1} r}{2}\leq z\leq -\sigma^{2m-1} r+\frac{\sigma}{2}\\
\left(\frac{\sigma^{2m}r}{2}-\sigma z\right)\left(1-\frac{1}{\sigma^{2(m-1)}r}\right)^{-1}\leq x\leq \frac{\sigma^{2m}r}{2}\qquad\textrm{if } \frac{\sigma^{2m-1} r}{2}\leq z\leq \frac{\sigma}{2}\\
\end{cases};
\end{align*}
we obtain
\begin{align*}
d\expe{\phi_d^1(X, Z)\indicator{R_1}{X, Z}} = o(1).
\end{align*}
For $\phi_d^2$, we have
\begin{align*}
A_3 \cap C_1=\begin{cases}
\sigma^2/2-\sigma z \leq x\leq -\sigma z +\sigma^2/2+\sigma^{2m}r/2\qquad\textrm{if } z<\sigma/2 - \sigma^{2m-1} r/2\\
\sigma^{2m}r/2 < x\leq -\sigma z +\sigma^2/2+\sigma^{2m}r/2\qquad\textrm{if } \sigma/2 - \sigma^{2m-1}r/2\leq z\leq \sigma/2
\end{cases},
\end{align*}
and
\begin{align*}
\expe{\left(\frac{\sigma^2}{2}-\sigma Z\right)\indicator{A_3}{X}\indicator{C_1}{X, Z}} 
&=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2 - \sigma^{2m-1} r/2}e^{-z^2/2}[\\
&\qquad\qquad\frac{\sigma^3}{6}\begin{cases}
-3rz \qquad \textrm{if } m= 1\\
0\qquad \textrm{if } m> 1\\
\end{cases} \\
&\qquad+ \dots]\rmd z+ o(1).
\end{align*}
Similarly, we obtain
\begin{align*}
A_3\cap C_2=\begin{cases}
\sigma^2/2-\sigma z-\sigma^{2m}r/2\leq x\leq \sigma^2/2-\sigma z\qquad\textrm{if } z< \sigma/2-\sigma^{2m-1} r\\
\sigma^{2m}r/2< x\leq \sigma^2/2-\sigma z\qquad\textrm{if } \sigma/2-\sigma^{2m-1} r< z<
	\sigma/2 - \sigma^{2m-1} r/2
\end{cases}
\end{align*}
and
\begin{align*}
\expe{\left(2X-\frac{\sigma^2}{2}+\sigma Z\right)\indicator{A_3}{X}\indicator{C_2}{X, Z}}
&=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2-\sigma^{2m-1} r}e^{-z^2/2}[\\
&\qquad\qquad\frac{\sigma^3}{6}\begin{cases}
-3rz \qquad \textrm{if } m= 1\\
0\qquad \textrm{if } m> 1\\
\end{cases} \\
&\qquad+ \dots]\rmd z+ o(1).
\end{align*}
Finally, 
\begin{align*}
A_3\cap (C_1\cup C_2)=\begin{cases}
\sigma^{2m}r/2\leq x\leq \sigma^{2m}r/2+\sigma^2/2-\sigma z\qquad\textrm{if } \sigma/2- \sigma^{2m-1} r\leq z\leq \sigma/2\\
-\sigma^{2m}r/2+\sigma^2/2-\sigma z< x\leq \sigma^{2m}r/2+\sigma^2/2-\sigma z\qquad\textrm{if } z< \sigma/2- \sigma^{2m-1} r
\end{cases},
\end{align*}
and
\begin{align*}
&\expe{\left(\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X+\left(1-\frac{1}{\sigma^{2(m-1)}r}\right)\left(\frac{\sigma^2}{2}-\sigma Z\right)\right)^2\right)\indicator{A_3}{X}\indicator{C_1\cup C_2}{X, Z}}\\
&\qquad\qquad=\frac{1}{2\sqrt{2\uppi}}\int ^{ \sigma/2- \sigma^{2m-1} r}_{-\infty}e^{-z^2/2}[\\
&\qquad\qquad\frac{\sigma^3}{6}\begin{cases}
3rz \qquad \textrm{if } m= 1\\
0\qquad \textrm{if } m> 1\\
\end{cases} \\
&\qquad+ \dots]\rmd z + o(1).
\end{align*}
For $\phi_d^3$, we have, in the case $r\geq \sigma^{-2(m-1)}$,
\begin{align*}
A_1\cap B_3&=\begin{cases}
0\leq x\leq \frac{\sigma^{2m}r}{2}\qquad\textrm{if }  z> \frac{\sigma^{2m-1} r}{2}\\
\left(\frac{\sigma^{2m}r}{2}-\sigma z\right)\left(1-\frac{1}{\sigma^{2(m-1)}r}\right)^{-1}< x\leq \frac{\sigma^{2m}r}{2}\qquad\textrm{if } \frac{\sigma}{2}\leq z\leq \frac{\sigma^{2m-1} r}{2}
\end{cases},\\
A_1\cap B_4&=\begin{cases}
0\leq x\leq \frac{\sigma^{2m}r}{2}\qquad\textrm{if } z< \frac{\sigma}{2}-\sigma^{2m-1} r\\
0\leq  x<\left(\frac{\sigma^{2m}r}{2}-\sigma z\right)\left(1-\frac{1}{\sigma^{2(m-1)}r}\right)^{-1}\qquad\textrm{if } \frac{\sigma}{2}-\sigma^{2m-1} r\leq z\leq -\frac{\sigma^{2m-1} r}{2}
\end{cases};
\end{align*}
from which we obtain
\begin{align*}
&\expe{\left(\frac{1}{\sigma^{2(m-1)}r}X-\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X -\sigma Z+\frac{\sigma^2}{2}\right)^2\right)\indicator{A_1}{X}\indicator{ B_3}{X, Z}} \\
&\qquad\qquad=\frac{1}{2\sqrt{2\uppi}}\int_{\sigma^{2m-1} r/2}^{+\infty}e^{-z^2/2}[\\
&\qquad\qquad\frac{\sigma^3}{6}\begin{cases}
-\frac{3}{4}rz \qquad \textrm{if } m= 1\\
0\qquad \textrm{if } m> 1\\
\end{cases} \\
&\qquad+ \dots]\rmd z + o(1),\\
&\expe{\left(2X-\frac{1}{\sigma^{2(m-1)}r}X+\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X -\sigma Z-\frac{\sigma^2}{2}\right)^2\right)\indicator{A_1}{X}\indicator{ B_4}{X, Z}} \\
&\qquad\qquad=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2-\sigma^{2m-1} r/2}e^{-z^2/2}[\\
&\qquad\qquad\frac{\sigma^3}{6}\begin{cases}
\frac{9}{4}rz \qquad \textrm{if } m= 1\\
0\qquad \textrm{if } m> 1\\
\end{cases} \\
&\qquad+ \dots]\rmd z + o(1).
\end{align*}
For the case $0\leq r<\sigma^{-2(m-1)}$, proceeding as above, we find that
\begin{align*}
A_1\cap B_3&=\begin{cases}
0\leq x\leq \frac{\sigma^{2m}r}{2}\qquad\textrm{if } z> \frac{\sigma}{2}\\
0\leq  x<\left(\frac{\sigma^{2m}r}{2}-\sigma z\right)\left(1-\frac{1}{\sigma^{2(m-1)}r}\right)^{-1}\qquad\textrm{if } \frac{\sigma^{2m-1} r}{2}\leq z\leq \frac{\sigma}{2}
\end{cases},\\
A_1\cap B_4&=\begin{cases}
0\leq x\leq \frac{\sigma^{2m}r}{2}\qquad\textrm{if } z< -\frac{\sigma^{2m-1} r}{2}\\
\left(-\frac{\sigma^{2m}r}{2}-\sigma z\right)\left(1-\frac{1}{\sigma^{2(m-1)}r}\right)^{-1}<x\leq \frac{\sigma^{2m}r}{2}\qquad\textrm{if } -\frac{\sigma^{2m-1} r}{2}\leq z\leq -\sigma^{2m-1} r+\frac{\sigma}{2}
\end{cases};
\end{align*}
and the corresponding expectations are
\begin{align*}
&\expe{\left(\frac{1}{\sigma^{2(m-1)}r}X-\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X -\sigma Z+\frac{\sigma^2}{2}\right)^2\right)\indicator{A_1}{X}\indicator{ B_3}{X, Z}} \\
&\qquad\qquad=\frac{1}{2\sqrt{2\uppi}}\int_{\sigma/2}^{+\infty}e^{-z^2/2}[\\
&\qquad\qquad\frac{\sigma^3}{6}\begin{cases}
-\frac{3}{4}rz \qquad \textrm{if } m= 1\\
0\qquad \textrm{if } m> 1\\
\end{cases} \\
&\qquad+ \dots]\rmd z + o(1),\\
&\expe{\left(2X-\frac{1}{\sigma^{2(m-1)}r}X+\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X -\sigma Z-\frac{\sigma^2}{2}\right)^2\right)\indicator{A_1}{X}\indicator{ B_4}{X, Z}} \\
&\qquad\qquad=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{-\sigma^{2m-1} r/2}e^{-z^2/2}[\\
&\qquad\qquad\frac{\sigma^3}{6}\begin{cases}
\frac{9}{4}rz \qquad \textrm{if } m= 1\\
0\qquad \textrm{if } m> 1\\
\end{cases} \\
&\qquad+ \dots]\rmd z + o(1).
\end{align*}
Finally, consider $\phi_d^4$ and $A_3 \cap  C_4=\left\lbrace z<\frac{\sigma}{2}-\sigma^{2m-1} r, \frac{\sigma^{2m}r}{2}<x\leq \frac{\sigma^2}{2 }-\sigma z -\frac{\sigma^{2m}r}{2}\right\rbrace$, then
\begin{align*}
    \expe{\left(2X-\frac{\sigma^2}{2}+\sigma Z\right)\indicator{A_3}{X}\indicator{ C_4}{X, Z}}
&=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2-\sigma^{2m-1} r}e^{-z^2/2}\left[\frac{\sigma^3}{6}z^3+ \dots\right]\rmd z.
\end{align*}

\subsubsection{Second Moment}
\paragraph{Case (a):} $m=1/2$

For $\phi_d^1$ and $r\geq \sigma$ we have
\begin{align*}
\expe{\left(\frac{\sigma}{r}X-\sigma Z\right)^2\indicator{A_1}{X}\indicator{B_1}{X, Z}} &= \frac{1}{2\sqrt{2\uppi}}\int_{ \sigma/2}^{r/2}e^{-z^2/2}\left[\frac{\sigma^3}{6}(3z^2r-6z^3)+\dots\right]\rmd z\\
&+ \frac{1}{2\sqrt{2\uppi}}\int_{ \sigma/2-r/2}^{0}e^{-z^2/2}\left[\frac{\sigma^3}{2}(2z^3+rz^2)+\dots\right]\rmd z+o(1),\\
\expe{\left(2X-\frac{\sigma}{r}X+\sigma Z\right)^2\indicator{A_1}{X}\indicator{B_2}{X, Z}} &= \frac{1}{2\sqrt{2\uppi}}\int_{ \sigma/2-r/2}^{0}e^{-z^2/2}\left[-\frac{\sigma^3z^3}{3}+\dots\right]\rmd z\\
&+ \frac{1}{2\sqrt{2\uppi}}\int_{ \sigma/2-r}^{-r/2}e^{-z^2/2}\left[\frac{\sigma^2}{0}\cdot 0+\dots\right]\rmd z+o(1),
\end{align*}

For $\phi_d^2$, we have
\begin{align*}
\expe{\left(\frac{\sigma^2}{2}-\sigma Z\right)^2\indicator{A_3}{X}\indicator{C_1}{X, Z}} 
&=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2 -  r/2}e^{-z^2/2}\\
&\qquad\qquad\left[\frac{\sigma^3}{2}rz^2+\frac{\sigma^3}{8}r(rz-4z^2+2)+...\right]\rmd z\\
&+\frac{1}{2\sqrt{2\uppi}}\int_{\sigma/2 -  r/2}^{\sigma/2} e^{-z^2/2}\\
&\qquad\qquad\left[-\sigma^3 z^3+...\right]\rmd z,\\
\expe{\left(2X-\frac{\sigma^2}{2}+\sigma Z\right)^2\indicator{A_3}{X}\indicator{C_2}{X, Z}}
&=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2- r}e^{-z^2/2}\\
&\qquad\qquad\left[\frac{\sigma^3}{6}r (r^2 + 3r z + 3 z^2)+...\right]\rmd z\\
&+\frac{1}{2\sqrt{2\uppi}}\int_{\sigma/2- r}^{\sigma/2-r/2}e^{-z^2/2}\\
&\qquad\qquad\left[\frac{\sigma^3}{6}(-r^3-3r^2z-3rz^2-2z^3)+...\right]\rmd z.
\end{align*}
and
\begin{align*}
&\expe{\left(\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{\sigma}{r}X+\left(1-\frac{\sigma}{r}\right)\left(\frac{\sigma^2}{2}-\sigma Z\right)\right)^2\right)^2\indicator{A_3}{X}\indicator{C_1\cup C_2}{X, Z}}\\
&\qquad\qquad=\frac{1}{2\sqrt{2\uppi}}\int_{\sigma/2- r}^{\sigma/2}e^{-z^2/2}\\
&\qquad\qquad\qquad\left[+...\right]\rmd z\\
&\qquad\qquad+\frac{1}{2\sqrt{2\uppi}}\int ^{ \sigma/2- r}_{-\infty}e^{-z^2/2}\\
&\qquad\qquad\qquad\left[+...\right]\rmd z.
\end{align*}
For $\phi_d^3$ we obtain
\begin{align*}
&\expe{\left(\frac{\sigma}{r}X-\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{\sigma}{r}X -\sigma Z+\frac{\sigma^2}{2}\right)^2\right)^2\indicator{A_1}{X}\indicator{ B_3}{X, Z}} \\
&\qquad\qquad=\frac{1}{2\sqrt{2\uppi}}\int_{ r/2}^{+\infty}e^{-z^2/2}\left[\frac{\sigma^3}{24}rz^2+...\right]\rmd z\\
&\qquad\qquad+\frac{1}{2\sqrt{2\uppi}}\int_{ \sigma/2}^{r/2}e^{-z^2/2}\left[+...\right]\rmd z,\\
&\expe{\left(2X-\frac{\sigma}{r}X+\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{\sigma}{r}X -\sigma Z-\frac{\sigma^2}{2}\right)^2\right)^2\indicator{A_1}{X}\indicator{ B_4}{X, Z}} \\
&\qquad\qquad=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2- r}e^{-z^2/2}\left[+...\right]\rmd z\\
&\qquad\qquad+\frac{1}{2\sqrt{2\uppi}}\int^{-r/2}_{\sigma/2- r}e^{-z^2/2}\left[+...\right]\rmd z.
\end{align*}
Finally, for $\phi_d^4$ we have
\begin{align*}
    \expe{\left(2X-\frac{\sigma^2}{2}+\sigma Z\right)^2\indicator{A_3}{X}\indicator{ C_4}{X, Z}}
&=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2- r}e^{-z^2/2}\left[-\frac{\sigma^3}{3}
(r+z)^3+ \dots\right]\rmd z.
\end{align*}
\paragraph{Case (b):} $m\geq 1$

Following the same approach taken for the first moment, we find that $\expe{\phi_d^1(X, Z)^2\indicator{R_1}{X, Z}} = o(1)$. Then, we have for $\phi_d^2$
\begin{align*}
&\expe{\left(\frac{\sigma^2}{2}-\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X-\left(1-\frac{1}{\sigma^{2(m-1)}r}\right)\left(\frac{\sigma^2}{2}+\sigma Z\right)\right)^2\right)^2\indicator{A_3}{X}\indicator{C_1}{X, Z}} \\
&\quad+\expe{\left(2X-\frac{\sigma^2}{2}+\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X-\left(1-\frac{1}{\sigma^{2(m-1)}r}\right)\left(\frac{\sigma^2}{2}+\sigma Z\right)\right)^2\right)^2\indicator{A_3}{X}\indicator{C_2}{X, Z}}\\
&\qquad = \expe{\left(\frac{\sigma^2}{2}-\sigma Z\right)^2\indicator{A_3}{X}\indicator{C_1}{X, Z}} + \expe{\left(2X-\frac{\sigma^2}{2}+\sigma Z\right)^2\indicator{A_3}{X}\indicator{C_2}{X, Z}} \\
&\qquad + 2\expe{\left(\frac{\sigma^2}{2}-\sigma Z\right)\left(\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X+\left(1-\frac{1}{\sigma^{2(m-1)}r}\right)\left(\frac{\sigma^2}{2}-\sigma Z\right)\right)^2\right)\indicator{A_3}{X}\indicator{C_1}{X, Z}}\\
&\qquad + 2\expe{\left(2X-\frac{\sigma^2}{2}+\sigma Z\right)\left(\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X+\left(1-\frac{1}{\sigma^{2(m-1)}r}\right)\left(\frac{\sigma^2}{2}-\sigma Z\right)\right)^2\right)\indicator{A_3}{X}\indicator{C_2}{X, Z}} \\
&\qquad + \expe{\left(\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X+\left(1-\frac{1}{\sigma^{2(m-1)}r}\right)\left(\frac{\sigma^2}{2}-\sigma Z\right)\right)^2\right)^2\indicator{A_3}{X}\indicator{C_1\cup C_2}{X, Z}} \\
&\qquad=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2-\sigma^{2m-1} r/2}e^{-z^2/2}\left[\frac{\sigma^3}{6}\ 0+...\right]\rmd z+ \frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2 - \sigma^{2m-1} r}e^{-z^2/2}\left[\frac{\sigma^3}{6}\ 0+...\right]\rmd z\\
&\qquad +\frac{1}{\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2-\sigma^{2m-1} r/2}e^{-z^2/2}\left[\frac{\sigma^3}{6}\ 0+...\right]\rmd z+ \frac{1}{\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2 - \sigma^{2m-1} r}e^{-z^2/2}\left[\frac{\sigma^3}{6}\ 0+...\right]\rmd z\\
&\qquad \frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2 - \sigma^{2m-1} r}e^{-z^2/2}\left[\frac{\sigma^3}{6}\ 0+...\right]\rmd z + o(1).\\
\end{align*}
For $\phi_d^3$, in the case $r\geq \sigma^{-2(m-1)}$ we have
\begin{align*}
&\expe{\left(\frac{1}{\sigma^{2(m-1)}r}X-\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X -\sigma Z+\frac{\sigma^2}{2}\right)^2\right)^2\indicator{A_1}{X}\indicator{ B_3}{X, Z}} \\
&\qquad\qquad=\frac{1}{2\sqrt{2\uppi}}\int_{\sigma^{2m-1} r/2}^{+\infty}e^{-z^2/2}\left[\frac{\sigma^3}{6}\ 0+...\right] \rmd z + o(1)\\
&\expe{\left(2X-\frac{1}{\sigma^{2(m-1)}r}X+\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X -\sigma Z-\frac{\sigma^2}{2}\right)^2\right)^2\indicator{A_1}{X}\indicator{ B_4}{X, Z}} \\
&\qquad\qquad=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2-\sigma^{2m-1} r/2}e^{-z^2/2}\left[\frac{\sigma^3}{6}\ 0+...\right] \rmd z + o(1).
\end{align*}
Similarly, in the case $0\leq r< \sigma^{-2(m-1)}$ we obtain
\begin{align*}
&\expe{\left(\frac{1}{\sigma^{2(m-1)}r}X-\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X -\sigma Z+\frac{\sigma^2}{2}\right)^2\right)^2\indicator{A_1}{X}\indicator{ B_3}{X, Z}} \\
&\qquad\qquad=\frac{1}{2\sqrt{2\uppi}}\int_{\sigma/2}^{+\infty}e^{-z^2/2}\left[\frac{\sigma^3}{6}\ 0+...\right] \rmd z + o(1)\\
&\expe{\left(2X-\frac{1}{\sigma^{2(m-1)}r}X+\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X -\sigma Z-\frac{\sigma^2}{2}\right)^2\right)^2\indicator{A_1}{X}\indicator{ B_4}{X, Z}} \\
&\qquad\qquad=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{-\sigma^{2m-1} r/2}e^{-z^2/2}\left[\frac{\sigma^3}{6}\ 0+...\right] \rmd z + o(1).
\end{align*}
Finally, for $\phi_d^4$ we have
\begin{align*}
    \expe{\left(2X-\frac{\sigma^2}{2}+\sigma Z\right)^2\indicator{A_3}{X}\indicator{ C_4}{X, Z}}
&=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2-\sigma^{2m-1} r}e^{-z^2/2}\left[-\frac{z^3\sigma^3}{3}+...\right]\rmd z.
\end{align*}
\subsubsection{Third Moment}
\paragraph{Case (a):} $m=1/2$
%For $\phi_d^2$, we have
%\begin{align*}
%\expe{\left(\frac{\sigma^2}{2}-\sigma Z\right)^3\indicator{A_3}{X}\indicator{C_1}{X, Z}} 
%&=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2 -  r/2}e^{-z^2/2}\\
%&\qquad\qquad\left[\sigma^4...\right]\rmd z\\
%&+\frac{1}{2\sqrt{2\uppi}}\int_{\sigma/2 -  r/2}^{\sigma/2} e^{-z^2/2}\\
%&\qquad\qquad\left[\sigma^4+...\right]\rmd z,
%\end{align*}
%and
%\begin{align*}
%\expe{\left(2X-\frac{\sigma^2}{2}+\sigma Z\right)^3\indicator{A_3}{X}\indicator{C_2}{X, Z}}
%&=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2- r}e^{-z^2/2}\\
%&\qquad\qquad\left[\sigma^4+...\right]\rmd z\\
%&+\frac{1}{2\sqrt{2\uppi}}\int_{\sigma/2- r}^{\sigma/2-r/2}e^{-z^2/2}\\
%&\qquad\qquad\left[\sigma^4+...\right]\rmd z.
%\end{align*}
%Finally, for $\phi_d^4$ we have
%\begin{align*}
%    \expe{\left(2X-\frac{\sigma^2}{2}+\sigma Z\right)^3\indicator{A_3}{X}\indicator{ C_4}{X, Z}}
%&=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2- r}e^{-z^2/2}\left[\frac{\sigma^3}{6}\cdot 0
%+ \dots\right]\rmd z.
%\end{align*}

\paragraph{Case (b):} $m\geq 1$


Proceeding as above, we find that $\expe{\phi_d^1(X, Z)^3\indicator{R_1}{X, Z}} = o(1)$. Then, using H\"older's inequality for $\phi_d^2$, we have
\begin{align*}
&\expe{\left(\frac{\sigma^2}{2}-\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X+\left(1-\frac{1}{\sigma^{2(m-1)}r}\right)\left(\frac{\sigma^2}{2}-\sigma Z\right)\right)^2\right)^3\indicator{A_3}{X}\indicator{C_1}{X, Z}} \\
&\qquad + \expe{\left(2X-\frac{\sigma^2}{2}+\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X+\left(1-\frac{1}{\sigma^{2(m-1)}r}\right)\left(\frac{\sigma^2}{2}-\sigma Z\right)\right)^2\right)^3\indicator{A_3}{X}\indicator{C_2}{X, Z}}\\
&\qquad\qquad\leq C \left(\expe{\left(\frac{\sigma^2}{2}-\sigma Z\right)^3\indicator{A_3}{X}\indicator{C_1}{X, Z}} +\expe{\left(2X-\frac{\sigma^2}{2}+\sigma Z\right)^3\indicator{A_3}{X}\indicator{C_2}{X, Z}}\right)\\
&\qquad\qquad + C \expe{\left(\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X+\left(1-\frac{1}{\sigma^{2(m-1)}r}\right)\left(\frac{\sigma^2}{2}-\sigma Z\right)\right)^2\right)^3\indicator{A_3}{X}\indicator{C_1\cup C_2}{X, Z}}\\
&\qquad\qquad = \frac{C}{2\sqrt{2\uppi}}\left(\int_{-\infty}^{\sigma/2 - \sigma^{2m-1} r/2}e^{-z^2/2}\left[-\frac{\sigma^3}{6}\cdot 0+...\right]\rmd z+\int_{-\infty}^{\sigma/2-\sigma^{2m-1} r}e^{-z^2/2}\left[-\frac{\sigma^3}{6}\cdot 0+...\right]\rmd z\right)\\
&\qquad\qquad + \frac{C}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2-\sigma^{2m-1} r}e^{-z^2/2}\left[\frac{\sigma^3}{6}\cdot 0+...\right]\rmd z +o(1).
\end{align*}
For $\phi_d^3$, in the case $r \geq \sigma^{-2(m-1)}$ we have, using again H\"older's inequality,
\begin{align*}
&\expe{\left(\frac{1}{\sigma^{2(m-1)}r}X-\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X -\sigma Z+\frac{\sigma^2}{2}\right)^2\right)^3\indicator{A_1}{X}\indicator{ B_3}{X, Z}} \\
&\qquad\qquad=\frac{1}{2\sqrt{2\uppi}}\int_{\sigma^{2m-1} r/2}^{+\infty}e^{-z^2/2}\left[-\frac{\sigma^3}{6}\cdot 0+...\right] \rmd z + o(1)\\
&\expe{\left(2X-\frac{1}{\sigma^{2(m-1)}r}X+\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X -\sigma Z-\frac{\sigma^2}{2}\right)^2\right)^3\indicator{A_1}{X}\indicator{ B_4}{X, Z}} \\
&\qquad\qquad\leq C\expe{\left(2X-\frac{1}{\sigma^{2(m-1)}r}X+\sigma Z\right)^3\indicator{A_1}{X}\indicator{ B_4}{X, Z}} \\
&\qquad\qquad+ C\expe{\left(\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X -\sigma Z-\frac{\sigma^2}{2}\right)^2\right)^3\indicator{A_1}{X}\indicator{ B_4}{X, Z}} + o(1)\\
&\qquad\qquad = C\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{-\sigma^{2m-1} r/2}e^{-z^2/2}\left[\frac{\sigma^3}{6}\cdot 0+...\right] \rmd z + o(1).
\end{align*}
Similarly, in the case $0\leq r < \sigma^{-2(m-1)}$ we obtain
\begin{align*}
&\expe{\left(\frac{1}{\sigma^{2(m-1)}r}X-\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X -\sigma Z+\frac{\sigma^2}{2}\right)^2\right)^3\indicator{A_1}{X}\indicator{ B_3}{X, Z}} \\
&\qquad\qquad=\frac{1}{2\sqrt{2\uppi}}\int_{\sigma/2}^{+\infty}e^{-z^2/2}\left[-\frac{\sigma^3}{6}\cdot 0+...\right] \rmd z + o(1)\\
&\expe{\left(2X-\frac{1}{\sigma^{2(m-1)}r}X+\sigma Z+\frac{Z^2}{2}-\frac{1}{2\sigma^2}\left(\frac{1}{\sigma^{2(m-1)}r}X -\sigma Z-\frac{\sigma^2}{2}\right)^2\right)^3\indicator{A_1}{X}\indicator{ B_4}{X, Z}} \\
&\qquad\qquad=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{-\sigma^{2m-1} r/2}e^{-z^2/2}\left[\frac{\sigma^3}{6}\cdot 0++...\right] \rmd z + o(1).
\end{align*}
Finally, for $\phi_d^4$ we have
\begin{align*}
    \expe{\left(2X-\frac{\sigma^2}{2}+\sigma Z\right)^3\indicator{A_3}{X}\indicator{ C_4}{X, Z}}
&=\frac{1}{2\sqrt{2\uppi}}\int_{-\infty}^{\sigma/2-\sigma^{2m-1} r}e^{-z^2/2}\left[\frac{\sigma^3}{6}\cdot 0+...\right]\rmd z.
\end{align*}


==> sections_revision/prox_derivatives.tex <==
\section{Additional results for the proof of Theorem~\ref{theo:differentiable}}
\subsection{Derivatives of proximity map for differentiable targets}
\label{app:derivatives_prox}
\fral{We should decide if we want to keep this or just say we use matematica}

Recall that, in the differentiable case, $\prox_g^{\sigma^{2m}r/2}(x)=\frac{\sigma^{2m}r}{2} g^\prime(\prox_g^{\sigma^{2m}r/2}(x))+x$
then
\begin{align*}
&\frac{\partial}{\partial \sigma} \prox_g^{\sigma^{2m}r/2}(x)_{|\sigma =0} =\begin{cases} 
\frac{r}{2}g^{\prime}(x)\qquad \textrm{if } m= 1/2\\
0\qquad \textrm{if } m> 1/2\\
\infty \qquad \textrm{otherwise}
\end{cases}\\
&\frac{\partial^2}{\partial \sigma^2} \prox_g^{\sigma^{2m}r/2}(x)_{|\sigma =0} =\begin{cases}
\frac{r^2}{2}g^{\prime}(x)g^{\dprime}(x)\qquad \textrm{if } m = 1/2\\
rg^{\prime}(x)\qquad \textrm{if } m = 1\\
0 \qquad \textrm{if } m > 1\\
\infty \qquad \textrm{otherwise}
\end{cases}\\
&\frac{\partial^3}{\partial \sigma^3}\prox_g^{\sigma^{2m}r/2}(x)_{|\sigma =0} = 
\begin{cases}
\frac{3r^3}{8}g^{\dprime\prime}(x)\left[g^{\prime}(x)\right]^2+\frac{3r^3}{4}g^{\prime}(x)\left[g^{\dprime}(x)\right]^2\qquad \textrm{if } m = 1/2\\
3rg^{\prime}(x)\qquad \textrm{if } m = 3/2\\
0 \qquad \textrm{if }  m=1, m > 3/2\\
\infty \qquad \textrm{otherwise}
\end{cases}\\
&\frac{\partial^4}{\partial \sigma^4}\prox_g^{\sigma^{2m}r/2}(x)_{|\sigma =0} = 
\begin{cases}
<\infty\qquad \textrm{if } m = 1/2\\
6r^2g^{\prime}(x)g^{\dprime}(x)\qquad \textrm{if } m = 1\\
12rg^{\prime}(x)\qquad \textrm{if } m = 2\\
0 \qquad \textrm{if }m=3/2, m>2\\
\infty \qquad \textrm{otherwise}
\end{cases}\\
&\frac{\partial^5}{\partial \sigma^5}\prox_g^{\sigma^{2m}r/2}(x)_{|\sigma =0} = 
\begin{cases}
<\infty\qquad \textrm{if } m = 1/2\\
60rg^{\prime}(x)\qquad \textrm{if } m = 5/2\\
0 \qquad \textrm{if } m=1, m=3/2, m=2, m>5/2\\
\infty \qquad \textrm{otherwise}
\end{cases}\\
%&\frac{\partial^6}{\partial \sigma^6}\prox_g^{\sigma^{2m}r/2}(x)_{|\sigma =0}\\
%&\qquad = 
%\begin{cases}
%< \infty\qquad \textrm{if } m = 1/2\\
%90r^3 \left(g^\prime(x)\left[g^{\dprime}(x)\right]^2+\frac{1}{2}\left[g^{\prime}(x)\right]^2g^{\dprime\prime}(x)\right) \qquad \textrm{if } m = 1\\
%180r^2g^{\prime}(x)g^{\dprime}(x)\qquad \textrm{if } m = 3/2\\
%360rg^{\prime}(x)\qquad \textrm{if } m = 3\\
%0 \qquad \textrm{if }  m=2, m=5/2, m>3\\
%\infty \qquad \textrm{otherwise}
%\end{cases}\\
\end{align*}
and
\begin{align*}
&\frac{\partial}{\partial x} \prox_g^{\sigma^{2m}r/2}(x)_{|\sigma =0} =1,\qquad\qquad\qquad\frac{\partial^{(k)}}{\partial x^{(k)}} \prox_g^{\sigma^{2m}r/2}(x)_{|\sigma =0} =0,
\end{align*}
for all integers $k>1$.
For the mixed derivatives we have
\begin{align*}
&\frac{\partial^2}{\partial \sigma \partial x} \prox_g^{\sigma^{2m}r/2}(x)_{|\sigma =0} =\begin{cases}
\frac{r}{2}g^{\dprime}(x)\qquad\textrm{if } m= 1/2\\
0\qquad\textrm{if }  m>1/2\\
\infty\qquad\textrm{otherwise}
\end{cases}\\
&\frac{\partial^3}{\partial \sigma^2 \partial x} \prox_g^{\sigma^{2m}r/2}(x)_{|\sigma =0} =\begin{cases}
\frac{r^2}{2}\left[g^{\dprime}(x)\right]^2+\frac{r^2}{2}g^{\prime}(x)g^{\dprime\prime}(x)\qquad\textrm{if } m= 1/2\\
rg^{\dprime}(x)\qquad\textrm{if } m= 1\\
0\qquad\textrm{if }  m>1/2\\
\infty\qquad\textrm{otherwise}
\end{cases}\\
&\frac{\partial^4}{\partial \sigma^3 \partial x} \prox_g^{\sigma^{2m}r/2}(x)_{|\sigma =0} =\begin{cases}
<\infty \qquad\textrm{if } m= 1/2\\
3rg^{\dprime}(x)\qquad\textrm{if } m= 3/2\\
0\qquad\textrm{if }  m=1, m>3/2\\
\infty\qquad\textrm{otherwise}
\end{cases}\\
&\frac{\partial^5}{\partial \sigma^4 \partial x} \prox_g^{\sigma^{2m}r/2}(x)_{|\sigma =0} =\begin{cases}
<\infty \qquad\textrm{if } m= 1/2\\
6r^2\left(g^{\prime}(x)g^{\dprime\prime}(x)+\left[g^{\dprime}(x)\right]^2\right)\qquad\textrm{if } m= 1\\
12rg^{\dprime}(x)\qquad\textrm{if } m= 2\\
0\qquad\textrm{if }  m=3/2, m>2\\
\infty\qquad\textrm{otherwise}
\end{cases}\\
\end{align*}
and
\begin{align*}
&\frac{\partial^3}{\partial \sigma\partial x^2 } \prox_g^{\sigma^{2m}r/2}(x)_{|\sigma =0} =\begin{cases}
\frac{r}{2}g^{\dprime\prime}(x) \qquad\textrm{if } m= 1/2\\
0\qquad\textrm{if }  m>1/2\\
\infty\qquad\textrm{otherwise}
\end{cases}\\
&\frac{\partial^4}{\partial \sigma\partial x^3 } \prox_g^{\sigma^{2m}r/2}(x)_{|\sigma =0} =\begin{cases}
<\infty \qquad\textrm{if } m= 1/2\\
0\qquad\textrm{if }  m>1/2\\
\infty\qquad\textrm{otherwise}
\end{cases}\\
&\frac{\partial^4}{\partial \sigma^2\partial x^2 } \prox_g^{\sigma^{2m}r/2}(x)_{|\sigma =0} =\begin{cases}
<\infty \qquad\textrm{if } m= 1/2\\
rg^{\dprime\prime}(x) \qquad\textrm{if } m= 1\\
0\qquad\textrm{if }  m>1/2\\
\infty\qquad\textrm{otherwise}
\end{cases}\\
&\frac{\partial^5}{\partial \sigma^3\partial x^2 } \prox_g^{\sigma^{2m}r/2}(x)_{|\sigma =0} =\begin{cases}
<\infty \qquad\textrm{if } m= 1/2\\
3rg^{\dprime\prime}(x) \qquad\textrm{if } m= 3/2\\
0\qquad\textrm{if }  m=1, m>3/2\\
\infty\qquad\textrm{otherwise}
\end{cases}\\
&\frac{\partial^5}{\partial \sigma^2\partial x^3 } \prox_g^{\sigma^{2m}r/2}(x)_{|\sigma =0} =\begin{cases}
<\infty \qquad\textrm{if } m= 1/2\\
rg^{\textrm{iv}}(x) \qquad\textrm{if } m= 1\\
0\qquad\textrm{if }  m>1\\
\infty\qquad\textrm{otherwise}
\end{cases}
\end{align*}
Links for derivatives:
\begin{itemize}
\item w.r.t. $\sigma$ \href{https://www.wolframalpha.com/input?i=f\%28s\%29+\%3D+s\%5E\%282m\%29r\%2F2+g\%27\%28f\%28s\%29\%29+first+derivative+s\%3D0}{here}
\item mixed \href{https://www.wolframalpha.com/input?i=1\%2F\%281-s\%5E\%282m\%29r\%2F2+g\%28f\%28s\%29\%29\%29+first+derivative+at+s\%3D0}{here} and \href{https://www.wolframalpha.com/input?i=s\%5E\%282m\%29r\%2F2*g\%27\%28f\%28s\%29\%29*\%281-s\%5E\%282m\%29r\%2F2+g\%28f\%28s\%29\%29\%29\%5E\%28-3\%29+first+derivative+at+s\%3D0}{here}
\end{itemize}




%%%%%%% OLD STUFF
%Recall that $\prox_g^{c^2\sigma^2/(2\ell^2)}(x)=\frac{c^2\sigma^2}{2\ell^2} g^\prime(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))+x$
%then
%\begin{align*}
%&\frac{\partial}{\partial \sigma} \prox_g^{c^2\sigma^2/(2\ell^2)}(x)_{|\sigma =0} =0\\
%&\frac{\partial^2}{\partial \sigma^2} \prox_g^{c^2\sigma^2/(2\ell^2)}(x)_{|\sigma =0} =\frac{c^2}{\ell^2}g^{\prime}(x)\\
%&\frac{\partial^3}{\partial \sigma^3}\prox_g^{c^2\sigma^2/(2\ell^2)}(x)_{|\sigma =0} = 0\\
%&\frac{\partial^4}{\partial \sigma^4} \prox_g^{c^2\sigma^2/(2\ell^2)}(x)_{|\sigma =0} = 6\frac{c^4}{\ell^4} g^{\prime}(x)g^{\dprime}(x)\\
%&\frac{\partial^5}{\partial \sigma^5} \prox_g^{c^2\sigma^2/(2\ell^2)}(x)_{|\sigma =0} = 0\\
%&\frac{\partial^6}{\partial \sigma^6} \prox_g^{c^2\sigma^2/(2\ell^2)}(x)_{|\sigma =0} = 90\frac{c^6}{\ell^6}g^\prime(x)\left[g^{\dprime}(x)\right]^2+45\frac{c^6}{\ell^6}\left[g^{\prime}(x)\right]^2g^{\dprime\prime}(x)
%\end{align*}
%
%Other derivatives
%\begin{align*}
%\frac{\partial}{\partial \sigma} \prox_g^{c^2\sigma^2/(2\ell^2)}(x) &= \frac{c^2\sigma/l^2 g^{\prime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x)) }{1-\frac{c^2\sigma^2}{2l^2} g^{\dprime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))}\\
%\frac{\partial^2}{\partial \sigma^2} \prox_g^{c^2\sigma^2/(2\ell^2)}(x)  &=\frac{c^2}{\ell^2}\left[1-\frac{c^2\sigma^2}{2l^2} g^{\dprime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\right]^{-3}\times \left[ g^{\prime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\right.\\
%&\left.+\sigma^2\frac{c^2}{\ell^2} g^{\dprime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))g^{\prime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\right.\\
%&\left.+\frac{c^4}{\ell^4}\frac{\sigma^4}{2}g^{\dprime\prime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\left[g^{\prime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\right]^2\right.\\
%&\left.-\sigma^4\frac{3c^4}{4l^4}g^{\prime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\left[g^{\dprime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\right]^2\right]\\
%\frac{\partial^3}{\partial \sigma^3} \prox_g^{c^2\sigma^2/(2\ell^2)}(x) &=\frac{c^2}{\ell^2}\left[1-\frac{c^2\sigma^2}{2l^2} g^{\dprime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\right]^{-5}\times \left[ 6\frac{c^2\sigma}{\ell^2} g^{\prime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))g^{\dprime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\right.\\
%&\left.+\left(6\frac{c^2}{\ell^2}-6\frac{c^4}{\ell^4}\right)\sigma^3g^{\prime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\left[g^{\dprime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\right]^2\right.\\
%&\left.+\frac{9}{2}\frac{c^4}{\ell^4}\sigma^3g^{\dprime\prime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\left[g^{\prime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\right]^2\right.\\
%&\left. +\frac{c^6}{2l^6}\sigma^5g^{\textrm{iv}}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\left[g^{\prime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\right]^3\right.\\
%&\left.+\left(3\frac{c^6}{\ell^6}-6\frac{c^4}{\ell^4}\right)\sigma^5g^{\prime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\left[g^{\dprime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\right]^3\right.\\
%&\left.+\left(3\frac{c^2}{\ell^2}+6\frac{c^4}{\ell^4}-9\frac{c^6}{\ell^6}\right)\sigma^5g^{\dprime\prime}(\prox_g^{\sigma^2/2}(x))g^{\dprime}(\prox_g^{\sigma^2/2}(x))\left[g^{\prime}(\prox_g^{\sigma^2/2}(x))\right]^2\right.\\
%&\left.-\frac{c^8}{4l^{8}}\sigma^7g^{\textrm{iv}}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))g^{\dprime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\left[g^{\prime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\right]^3\right.\\
%&\left.+\left(\frac{3}{2}\frac{c^6}{\ell^6}-\frac{3}{4}\frac{c^8}{\ell^8}\right)\sigma^7g^{\prime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\left[g^{\dprime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\right]^4\right.\\
%&\left.+\frac{3}{4}\frac{c^4}{\ell^4}\sigma^7 \left[g^{\prime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\right]^3\left[g^{\dprime\prime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\right]^2\right.\\
%&\left.+\left(\frac{9}{8}\frac{c^8}{\ell^8}-\frac{3}{4}\frac{c^4}{\ell^4}-\frac{3}{2}\frac{c^6}{\ell^6}\right)\sigma^7g^{\dprime\prime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\left[g^{\prime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\right]^2\left[g^{\dprime}(\prox_g^{c^2\sigma^2/(2\ell^2)}(x))\right]^2\right]
%\end{align*}
%and \href{https://www.wolframalpha.com/input/?i=f\%28s\%29+\%3D+c^2s\%5E2\%2F\%282l\%29+g\%27\%28f\%28s\%29\%29+first+derivative+}{here}
%
%Moreover
%\begin{align*}
%&\frac{\partial}{\partial x} \prox_g^{c^2\sigma^2/(2\ell^2)}(x)_{|\sigma =0} =1\\
%&\frac{\partial^{(k)}}{\partial x^{(k)}} \prox_g^{c^2\sigma^2/(2\ell^2)}(x)_{|\sigma =0} =0
%\end{align*}
%since
%\begin{align*}
%    \frac{\partial}{\partial x} \prox_g^{c^2\sigma^2/(2\ell^2)}(x) =\frac{1}{1-\frac{c^2\sigma^2}{2\ell^2}g^{\dprime}\left(\prox_g^{c^2\sigma^2/(2\ell^2)}(x)\right)}
%\end{align*}
%

==> sections_revision/taylor.tex <==
\subsection{Taylor expansions of log-acceptance ratio}
\label{app:derivatives_R}
\subsubsection{$R_1$}
Define $R_1(x, z, \sigma) = g\left[x + \frac{\sigma^2}{2} g^{\prime}\left(\prox_{g}^{\sigma^{2m}r/2}(x) \right)+ \sigma z\right] - g(x)$. To obtain the Taylor expansion in Theorem~\ref{theo:differentiable} we need the following derivatives
\begin{align*}
 R_1(x, z, 0)&= 0,\\
 \frac{\partial R_1}{\partial \sigma}(x, z, \sigma)_{\mid \sigma=0} &=g^\prime(x)z,\\
\frac{\partial^2 R_1}{\partial \sigma^2}(x, z, \sigma)_{\mid \sigma=0} &=z^2g^{\dprime}(x)+\left[g^\prime(x)\right]^2,\\
\frac{\partial^3 R_1}{\partial \sigma^3}(x, z, \sigma)_{\mid \sigma=0}&= z^3g^{\dprime\prime}(x)+3g^\prime(x)g^{\dprime}(x)\left[z+\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma =0}\right],\\
\frac{\partial^4 R_1}{\partial \sigma^4}(x, z, \sigma)_{\mid \sigma=0} &= z^4g^{ \textrm{iv}}(x)+6z^2g^{\dprime\prime}(x)g^{\prime}(x)+3g^{\dprime}(x)\left[g^{\prime}(x)\right]^2+12z\left[g^{\dprime}(x)\right]^2\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma =0}\\
&+6g^\prime(x)\left[g^{\dprime}(x)\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma =0}+\left(\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma =0}\right)^2g^{\dprime\prime}(x)\right].
\end{align*}
In addition, for $m>1/2$ we will also use
\begin{align*}
\frac{\partial^5 R_1}{\partial \sigma^5}(x, z, \sigma)_{\mid \sigma=0} &=  z^5g^{ \textrm{v}}(x)+10z^3g^{\textrm{iv}}(x)g^{\prime}(x)+15zg^{\dprime\prime}(x)\left[g^{\prime}(x)\right]^2\\
&+30z\left[g^{\dprime}(x)\right]^2\frac{\partial^2}{\partial^2 \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma =0} + 10g^{\prime}(x)g^{\dprime}(x)\frac{\partial^3}{\partial^3 \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma =0},\\
\frac{\partial^6 R_1}{\partial \sigma^6}(x, z, \sigma)_{\mid \sigma=0} &=z^6g^{ \textrm{vi}}(x)+15z^4g^{\textrm{v}}(x)g^{\prime}(x)+45z^2g^{\textrm{iv}}(x)\left[g^{\prime}(x)\right]^2+15g^{\dprime\prime}(x)\left[g^{\prime}(x)\right]^3\\
&+90g^{\prime}(x)\left[g^{\dprime}(x)\right]^2\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma =0}
+90g^{\dprime}(x)g^{\dprime\prime}(x)\frac{\partial^2}{\partial \sigma^2}\prox_{g}^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\\
&+60zg^{\dprime}(x)\frac{\partial^3}{\partial \sigma^3}\prox_{g}^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\\
&+15g^{\prime}(x)\left(g^{\dprime}(x)\frac{\partial^4}{\partial \sigma^4}\prox_{g}^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+3\left[\frac{\partial^2}{\partial \sigma^2}\prox_{g}^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]^2g^{\prime\dprime}(x)\right).
\end{align*}
%and
%\begin{align*}
%\frac{\partial^5 R_1}{\partial \sigma^5}(x, z, \sigma)_{\mid \sigma=0} &=  z^5g^{ \textrm{v}}(x)+10z^3g^{\textrm{iv}}(x)g^{\prime}(x)+15zg^{\dprime\prime}(x)\left[g^{\prime}(x)\right]^2\\
%&+30\left[g^{\dprime}(x)\right]^2g^{\prime}(x)\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma =0}+30z^2g^{\dprime\prime}(x)g^{\dprime}(x)\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma =0}\\
%&+30zg^{\dprime}(x)\left[g^{\dprime}(x)\frac{\partial^2}{\partial^2 \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma =0}+\left(\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma =0}\right)^2g^{\dprime\prime}(x)\right] \\
%&+ 10g^{\prime}(x)\left[g^{\dprime}(x)\frac{\partial^3}{\partial^3 \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma =0}+\left(\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma =0}\right)^3g^{\textrm{iv}}(x)\right.\\
%&\left.\qquad+3\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma =0}\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma =0}g^{\dprime\prime}(x)\right]\\
%\frac{\partial^6 R_1}{\partial \sigma^6}(x, z, \sigma)_{\mid \sigma=0} &=z^6g^{ \textrm{vi}}(x)+15z^4g^{\textrm{v}}(x)g^{\prime}(x)+45z^2g^{\textrm{iv}}(x)\left[g^{\dprime}(x)\right]^2+15g^{\dprime\prime}(x)\left[g^{\dprime}(x)\right]^3\\
%&+180zg^{\dprime\prime}(x) g^{\prime}(x)g^{\dprime}(x)\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma =0}+90g^{\dprime}(x)\left[\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma =0}g^{\dprime}(x)\right]^2\\
%&+90g^{\dprime}(x)g^{\prime}(x)\left(\frac{\partial^2}{\partial \sigma^2}\prox_{g}^{\sigma^{2m}r/2}(x)g^{\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)+\left[\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x)\right]^2g^{\prime\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\right)\\
%&+60z^3g^{\textrm{iv}}(x)g^{\dprime}(x)\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma =0}\\
%&+90z^2g^{\dprime\prime}(t)6\left(\frac{\partial^2}{\partial \sigma^2}\prox_{g}^{\sigma^{2m}r/2}(x)g^{\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)+\left[\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x)\right]^2g^{\prime\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\right)\\
%&+60zg^{\dprime}(x)\left(\frac{\partial^3}{\partial \sigma^3}\prox_{g}^{\sigma^{2m}r/2}(x)g^{\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)+\left[\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x)\right]^3g^{\textrm{iv}}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\right.\\
%&\left.\qquad+3\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x)\frac{\partial^2}{\partial \sigma^2}\prox_{g}^{\sigma^{2m}r/2}(x)g^{\prime\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\right)\\
%&+15g^{\prime}(x)\left(\frac{\partial^4}{\partial \sigma^4}\prox_{g}^{\sigma^{2m}r/2}(x)g^{\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)+3\left[\frac{\partial^2}{\partial \sigma^2}\prox_{g}^{\sigma^{2m}r/2}(x)\right]^2g^{\prime\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\right.\\
%&\left.\qquad+\left[\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x)\right]^4g^{\textrm{v}}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\right.\\
%&\left.\qquad+4\frac{\partial^3}{\partial \sigma^3}\prox_{g}^{\sigma^{2m}r/2}(x)\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x)g^{\prime\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\right.\\
%&\left.\qquad + 6 \left[\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x)\right]^2\frac{\partial^2}{\partial \sigma^2}\prox_{g}^{\sigma^{2m}r/2}(x)g^{\textrm{iv}}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\right)\\
%\end{align*}
%where
%\begin{align*}
%    t & = x + \frac{\sigma^2}{2} g^{\prime}\left(\prox_{g}^{\sigma^{2m}r/2}(x) \right)+ \sigma z\\
%    t^\prime & = \sigma g^{\prime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)+\frac{\sigma^2}{2}g^{\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x) + z\\
%    t^{\dprime} & = g^{\prime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)+ 2\sigma g^{\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x)\\
%    &+\frac{\sigma^2}{2}g^{\dprime\prime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\left[\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x)\right]^2+\frac{\sigma^2}{2}g^{\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\frac{\partial^2}{\partial \sigma^2}\prox_{g}^{\sigma^{2m}r/2}(x)\\
%    t^{\dprime\prime} & = 3\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x)g^{\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\\
%    &+3\sigma \left(\frac{\partial^2}{\partial \sigma^2}\prox_{g}^{\sigma^{2m}r/2}(x)g^{\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)+3\left[\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x)\right]^2g^{\prime\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\right)\\
%    &+\frac{\sigma^2}{2}\left(\frac{\partial^3}{\partial \sigma^3}\prox_{g}^{\sigma^{2m}r/2}(x)g^{\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)+\left[\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x)\right]^3g^{\textrm{iv}}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\right.\\
%    &\left.\qquad+3\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x)\frac{\partial^2}{\partial \sigma^2}\prox_{g}^{\sigma^{2m}r/2}(x)g^{\prime\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\right)\\
%    t^{\textrm{iv}} &= 6\left(\frac{\partial^2}{\partial \sigma^2}\prox_{g}^{\sigma^{2m}r/2}(x)g^{\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)+\left[\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x)\right]^2g^{\prime\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\right)+o(1)\\
%     t^{\textrm{v}} &= 10\left(\frac{\partial^3}{\partial \sigma^3}\prox_{g}^{\sigma^{2m}r/2}(x)g^{\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)+\left[\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x)\right]^3g^{\textrm{iv}}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\right.\\
%&\left.\qquad+3\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x)\frac{\partial^2}{\partial \sigma^2}\prox_{g}^{\sigma^{2m}r/2}(x)g^{\prime\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\right)+o(1)\\
%     t^{\textrm{vi}} &= 15\left(\frac{\partial^4}{\partial \sigma^4}\prox_{g}^{\sigma^{2m}r/2}(x)g^{\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)+3\left[\frac{\partial^2}{\partial \sigma^2}\prox_{g}^{\sigma^{2m}r/2}(x)\right]^2g^{\prime\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\right.\\
%&\left.\qquad+\left[\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x)\right]^4g^{\textrm{v}}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)+4\frac{\partial^3}{\partial \sigma^3}\prox_{g}^{\sigma^{2m}r/2}(x)\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x)g^{\prime\dprime}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\right.\\
%&\left.\qquad + 6 \left[\frac{\partial}{\partial \sigma}\prox_{g}^{\sigma^{2m}r/2}(x)\right]^2\frac{\partial^2}{\partial \sigma^2}\prox_{g}^{\sigma^{2m}r/2}(x)g^{\textrm{iv}}\left(\prox_{g}^{\sigma^{2m}r/2}(x)\right)\right)+o(1)\\
%\end{align*}


%\href{https://www.wolframalpha.com/input/?i=g\%28f\%28s\%29\%29+sixth+derivative}{WOLFRAMALPHA}


\subsubsection{$R_2$}

Similarly to $R_1$, we obtain the derivatives of $R_2$:
\begin{align*}
R_2(x, z, 0)&= 0,\\
\frac{\partial R_2}{\partial \sigma}(x, z, \sigma)_{\vert \sigma =0} &= -z g^\prime(x),\\
\frac{\partial^2 R_2}{\partial \sigma^2}(x, z, \sigma)_{\vert \sigma =0} &= -\left[ g^\prime(x)\right]^2-zg^{\dprime}(x)\left[z+2\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right],\\
\frac{\partial^3 R_2}{\partial \sigma^3}(x, z, \sigma)_{\vert \sigma =0} &= -3g^{\prime}(x)g^{\dprime}(x)\left[z+2\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]\\
&-\frac{3}{2}z\left(\left[z+\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]^2g^{\dprime\prime}(x) \right.\\
&\left.+\left[g^{\prime}(x) +2z\frac{\partial^2}{\partial \sigma\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0} + \frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]g^{\dprime}(x) \right.\\
&\left. +\left[\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]^2 g^{\prime\dprime}(x)+\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}g^{\dprime}(x)\right),\\
\frac{\partial^4 R_2}{\partial \sigma^4}(x, z, \sigma)_{\vert \sigma =0} &= -3\left[g^{\dprime}(x)\right]^2\left[z+2\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]^2\\
&-6g^{\prime}(x)\left(\left[z+\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]^2g^{\dprime\prime}(x) \right.\\
&\left.+\left[g^{\prime}(x) +2z\frac{\partial^2}{\partial \sigma\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0} + \frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]g^{\dprime}(x) \right.\\
&\left. +\left[\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]^2 g^{\prime\dprime}(x)+\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}g^{\dprime}(x)\right)\\
&-2zg^{\textrm{iv}}(x)\left[z+\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]^3\\
&-6zg^{\dprime\prime}(x)\left[z+\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]\\
&\qquad\times\left[g^{\prime}(x)+2z\frac{\partial^2}{\partial \sigma\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]\\
&-2zg^{\dprime}(x)\left[3g^{\dprime}(x)\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+3g^{\prime}(x)\frac{\partial^2}{\partial \sigma\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right.\\
&\left.\qquad +3z^2\frac{\partial^3}{\partial \sigma\partial x^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+3z\frac{\partial^3}{\partial \sigma^2\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+\frac{\partial^3}{\partial \sigma^3}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]\\
&-2zg^{\textrm{iv}}(x)\left[\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]^3-6z\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}g^{\dprime\prime}(x)\\
&-2zg^{\dprime}(x)\frac{\partial^3}{\partial \sigma^3}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}.
\end{align*}
We then proceed to get the derivatives needed for $m>1/2$:
\begin{align*}
\frac{\partial^5 R_2}{\partial \sigma^5}(x, z, \sigma)_{\vert \sigma =0} &= -15zg^{\dprime}(x)\left(z^2g^{\dprime\prime}(x) +\left[g^{\prime}(x) +2\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]g^{\dprime}(x) \right)\\
&-5g^{\prime}(x)\left(2z^3g^{\textrm{iv}}(x)+6zg^{\dprime\prime}(x)\left[g^{\prime}(x)+\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]\right.\\
&\left.\qquad+2g^{\dprime}(x)\left[3z\frac{\partial^3}{\partial\sigma^2 \partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+\frac{\partial^3}{\partial \sigma^3}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]\right.\\
&\left.\qquad+2g^{\dprime}(x)\frac{\partial^3}{\partial \sigma^3}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right)\\
&-\frac{5}{2}g^{\textrm{v}}(x)z^5-\frac{5}{2}zg^{\dprime}(x)\frac{\partial^4}{\partial \sigma^4}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}- 15g^{\textrm{iv}}(x)z^3\left[g^{\prime}(x)+\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]\\
&-\frac{15}{2}zg^{\dprime\prime}(x)\left[g^{\prime}(x)+\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]^2-\frac{15}{2}zg^{\dprime\prime}(x)\left[\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]^2\\
&-10z^2 g^{\dprime\prime}(x)\left(3z\frac{\partial^3}{\partial \sigma^2\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+ \frac{\partial^3}{\partial \sigma^3}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right)\\
&-\frac{5}{2}zg^{\dprime}(x)
\left(\frac{\partial^4}{\partial \sigma^4}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+6g^{\dprime}(x)\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right.\\
&\qquad\left.+6g^{\prime}(x)\frac{\partial^3}{\partial \sigma^2\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+6z^2\frac{\partial^4}{\partial \sigma^2\partial x^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right.\\
&\left.\qquad+4z\frac{\partial^4}{\partial \sigma^3\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right)
\end{align*}
and
\begin{align*}
\frac{\partial^6 R_2}{\partial \sigma^6}(x, z, \sigma)_{\vert \sigma =0} &= -\frac{45}{2}\left(z^2g^{\dprime\prime}(x) +\left[g^{\prime}(x) +2\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]g^{\dprime}(x) \right)^2\\
&-15zg^{\dprime}(x)\left( 2z^3g^{\textrm{iv}}(x)+6zg^{\dprime\prime}(x)
\left[g^{\prime}(x)+\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]\right.\\
&\qquad+2g^{\dprime}(x)\left[3z\frac{\partial^3}{\partial\sigma^2 \partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+\frac{\partial^3}{\partial \sigma^3}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]\\
&\qquad\left.+2g^{\dprime}(x)\frac{\partial^3}{\partial \sigma^3}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right)\\
&-6g^{\prime}(x)A^{\textrm{v}} - zA^{\textrm{vi}},
\end{align*}
%To obtain higher order derivatives use the fact that $R_2=-\frac{1}{2}A^2$ with 
%\begin{align*}
%    A:=\left(\frac{\sigma}{2}g^\prime\left(\prox_g^{\sigma^{2m}r/2}\left[ \frac{\sigma^2}{2}g^\prime\left[\prox_g^{\sigma^{2m}r/2}(x)\right]+x+\sigma z\right]\right)+\frac{\sigma}{2}g^\prime\left[\prox_g^{\sigma^{2m}r/2}(x)\right]+ z\right)
%\end{align*}
%and  the derivatives of $A$ \href{https://www.wolframalpha.com/input/?i=s\%2F2g\%28f\%28s\%2C+u\%29\%29\%2Bz\%2Bs\%2F2g\%28f\%28s\%2C+s\%5E2\%2F2+g\%28f\%28s\%2C+u\%29\%29\%2Bu\%2Bsz\%29\%29\%2C+first+derivative+at+s\%3D0}{here}  where we defined $f(\sigma, x) := \prox_g^{\sigma^{2m}r/2}(x)$.
with
\begin{align*}
%    A^\prime &= g^\prime\left(x\right)\\
%    A^{\dprime} &=g^{\dprime}(x)\left[z+2\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]\\
%A^{\dprime\prime} &= \frac{3}{2}\left(\left[z+\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]^2g^{\dprime\prime}(x) \right.\\
%&\left.+\left[g^{\prime}(x) +2z\frac{\partial^2}{\partial \sigma\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0} + \frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]g^{\dprime}(x) \right.\\
%&\left. +\left[\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]^2 g^{\prime\dprime}(x)+\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}g^{\dprime}(x)\right)\\
%A^{\textrm{iv}} &= 2g^{\textrm{iv}}(x)\left[z+\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]^3\\
%&+6g^{\dprime\prime}(x)\left[z+\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]\left[g^{\prime}(x)+2z\frac{\partial^2}{\partial \sigma\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]\\
%&+2g^{\dprime}(x)\left[3g^{\dprime}(x)\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+3g^{\prime}(x)\frac{\partial^2}{\partial \sigma\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+3z^2\frac{\partial^3}{\partial \sigma\partial x^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right.\\
%&\left.\qquad +3z\frac{\partial^3}{\partial\sigma^2 \partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+\frac{\partial^3}{\partial \sigma^3}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]\\
%&+2g^{\textrm{iv}}(x)\left[\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]^3+6\frac{\partial^2}{\partial^2 \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\frac{\partial}{\partial \sigma}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}g^{\dprime\prime}(x)\\
%&+2g^{\dprime}(x)\frac{\partial^3}{\partial \sigma^3}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\\
A^{\textrm{v}} &= \frac{5}{2}g^{\textrm{v}}(x)z^4+\frac{5}{2}g^{\dprime}(x)\frac{\partial^4}{\partial \sigma^4}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+ 15g^{\textrm{iv}}(x)z^2\left[g^{\prime}(x)+\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]\\
&+\frac{15}{2}g^{\dprime\prime}(x)\left[g^{\prime}(x)+\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]^2+\frac{15}{2}g^{\dprime\prime}(x)\left[\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]^2\\
&+10z g^{\dprime\prime}(x)\left(3z\frac{\partial^3}{\partial \sigma^2\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+ \frac{\partial^3}{\partial \sigma^3}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right)\\
&+\frac{5}{2}g^{\dprime}(x)
\left(\frac{\partial^4}{\partial \sigma^4}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+6g^{\dprime}(x)\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+6g^{\prime}(x)\frac{\partial^3}{\partial \sigma^2\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right.\\
&\qquad\left.+6z^2\frac{\partial^4}{\partial \sigma^2\partial x^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+4z\frac{\partial^4}{\partial \sigma^3\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right),\\
A^{\textrm{vi}} &= 3\left(10g^{\dprime\prime}(x)\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\frac{\partial^3}{\partial \sigma^3}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+g^{\dprime}(x)\frac{\partial^5}{\partial \sigma^5}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+g^{\textrm{vi}}(x)z^5\right.\\
& + 10g^{\textrm{v}}(x)z^3\left[g^{\prime}(x)+\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right] + 15zg^{\textrm{iv}}(x)\left[g^{\prime}(x)+\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]^2\\
&+ 10g^{\textrm{iv}}(x)z^2\left[\frac{\partial^3}{\partial \sigma^3}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+3z\frac{\partial^3}{\partial \sigma^2\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]\\
&+ 10g^{\dprime\prime}(x)\left[g^{\prime}(x)+\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]\left[\frac{\partial^3}{\partial \sigma^3}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+3z\frac{\partial^3}{\partial \sigma^2\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]\\
&+5g^{\dprime\prime}(x)z\left[6g^{\dprime}(x)\frac{\partial^2}{\partial \sigma^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+6g^{\prime}(x)\frac{\partial^3}{\partial \sigma^2\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right.\\
&\qquad\left. +6z^2\frac{\partial^4}{\partial \sigma^2\partial x^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+3z\frac{\partial^4}{\partial \sigma^3\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+\frac{\partial^4}{\partial \sigma^4}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]\\
&+g^{\dprime}(x)\left[10g^{\dprime}(x)\frac{\partial^3}{\partial \sigma^3}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+10g^{\prime}(x)\frac{\partial^4}{\partial \sigma^3\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right.\\
&\qquad +5z\frac{\partial^5}{\partial \sigma^4\partial x}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+10z^2\frac{\partial^5}{\partial \sigma^3\partial x^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+10z^3\frac{\partial^5}{\partial \sigma^2\partial x^3}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\\
&\qquad\left.\left. +30g^{\prime}(x)z\frac{\partial^4}{\partial \sigma^2\partial x^2}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}+\frac{\partial^5}{\partial \sigma^5}\prox_g^{\sigma^{2m}r/2}(x)_{\mid \sigma=0}\right]\right).
\end{align*}

